Hierarchical clustering with maximum density paths and mixture models

Hierarchical clustering is an effective, interpretable method for analyzing structure in data. It reveals insights at multiple scales without requiring a predefined number of clusters and captures nested patterns and subtle relationships, which are often missed by flat clustering approaches. However, existing hierarchical clustering methods struggle with high-dimensional data, especially when there are no clear density gaps between modes. In this work, we introduce t-NEB, a probabilistically grounded hierarchical clustering method, which yields state-of-the-art clustering performance on naturalistic high-dimensional data. t-NEB consists of three steps: (1) density estimation via overclustering; (2) finding maximum density paths between clusters; (3) creating a hierarchical structure via bottom-up cluster merging. t-NEB uses a probabilistic parametric density model for both overclustering and cluster merging, which yields both high clustering performance and a meaningful hierarchy, making it a valuable tool for exploratory data analysis. Code is available at https://github.com/ecker-lab/tneb clustering.

==> figures/3d_plot/energy_plot_3d.tex <==
% \begin{figure}
\begin{wrapfigure}[7]{r}{0.5\linewidth}
    \centering
    \vspace{-12pt}
    \begin{subfigure}[b]{0.33\linewidth}
        \includegraphics[width=\textwidth]{figures/3d_plot/crop_energy_landscape_level_-5.png}
        % \caption{6 clusters}%, threshold -5}
        % \label{fig:level-5}
    \end{subfigure}%
    % \begin{subfigure}[b]{0.25\linewidth}
    %     \includegraphics[width=\textwidth]{figures/3d_plot/crop_energy_landscape_level_-6.3.png}
    %     % \caption{4 clusters}%, threshold -6.3}
    %     % \label{fig:level-6.3}
    % \end{subfigure}%
    \begin{subfigure}[b]{0.33\linewidth}
        \includegraphics[width=\textwidth]{figures/3d_plot/crop_energy_landscape_level_-7.png}
        % \caption{3 clusters}%, threshold -7}
        % \label{fig:level-7}
    \end{subfigure}%
    \begin{subfigure}[b]{0.33\linewidth}
        \includegraphics[width=\textwidth]{figures/3d_plot/crop_energy_landscape_level_-8.3.png}
        % \caption{2 clusters}%, threshold -8.3}
        % \label{fig:level-8.3}
    \end{subfigure}
    \caption{Density landscape thresholded at different ``water levels'' leading to 6, 3, and 2 clusters.}
    \label{fig:energy-landscapes}
    % \mrinline{check positive vs negative threshold}
\end{wrapfigure}
% \end{figure}
